Saying Hello World with MOLA - A Solution to the TTC 2011 Instructive Case

This paper describes the solution of Hello World transformations in MOLA transformation language. Transformations implementing the task are relatively straightforward and easily inferable from the task specification. The required additional steps related to model import and export are also described.

==> eptcsdata.tex <==
\providecommand{\firstpage}{237}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.21}{10.4204/EPTCS.74.21}}
\pdfoutput=1

